D3CODE: Disentangling Disagreements in Data across Cultures on Offensiveness Detection and Evaluation

While human annotations play a crucial role in language technologies, annotator subjectivity has long been overlooked in data collection. Recent studies that have critically examined this issue are often situated in the Western context, and solely document differences across age, gender, or racial groups. As a result, NLP research on subjectivity have overlooked the fact that individuals within demographic groups may hold diverse values, which can influence their perceptions beyond their group norms. To effectively incorporate these considerations into NLP pipelines, we need datasets with extensive parallel annotations from various social and cultural groups. In this paper we introduce the \dataset dataset: a large-scale cross-cultural dataset of parallel annotations for offensive language in over 4.5K sentences annotated by a pool of over 4k annotators, balanced across gender and age, from across 21 countries, representing eight geo-cultural regions. The dataset contains annotators' moral values captured along six moral foundations: care, equality, proportionality, authority, loyalty, and purity. Our analyses reveal substantial regional variations in annotators' perceptions that are shaped by individual moral values, offering crucial insights for building pluralistic, culturally sensitive NLP models.

==> sections/model.tex <==
%\subsection{Multi-Annotator Modeling}


\input{tabs/multi-perspective}
We follow a multi-task modeling approach proposed by \citet{davani2022dealing}, who implemented a multi-task model where each task is to predict a specific annotator's labels and all tasks sharing the same semantic representation of the items. 
Inspired by \citet{orlikowski-etal-2023-ecological}, we slightly change this approach to improve the scalability when the dataset includes thousands of annotators. To do so, we group annotators based on their similar perspectives and define each task as predicting a specific group's labels. 

We first perform an experiment with annotators' regions  their perspectives. In other words, we consider annotators from each gender, age, or region to provide one perspective about the data.

As discussed in our first analysis (refer) annotators' with similar moral values can have homogeneity in their perceptions regarding offensiveness. Therefore, we consider clustering annotators based on their similar moral values and test the multi-task modeling for predicting labels from each cluster. Similar to Analyses, we clustered annotators into six groups, and considered labels from each group as a perspective into the annotation task.



==> tabs/lexicon-long.tex <==
\begin{comment}
\begin{table*}[t]
\centering
\scalebox{.8}{
\begin{tabular}{lp{6.5cm}p{8.5
cm}}
\toprule
Group & Top 10 uniquely frequent words in offensive content & Uniquely offensive Instance \\\midrule
%Age, 18-30 & black, muslim, boy, people, right, think, allah, christian, good, kill \\
%Age, 30-50 & muslim, doing, allah, terrorist, country, canada, islamic, learn, thing, death \\
%Age, 50+ & jew, trump, christian, think, church, good, law, nazi, white, world \\
%\midrule
%Gender, Man & kill, allah, christian, quebec, bake, o, white, like, mosque, teach \\
%Gender, Woman & allah, mean, kill, good, news, transgendered, bake, quebec, o, thousand \\
%Gender, Other & government, problem, long, really, care, change, marriage, anti, new, point \\
%\midrule
Region, AC. & terrorist, trump, catholic, christian, white, anti, right, men, child, really & ``He was shouting God's name as he killed which is common for Islamic terrorists.. That might indicate his motivation'' \\
Region, ICS. & christian, men, church, child, feel, government, republican, probably, trump, transgendered & ``Fake Senator, Fake Tories, Fake Christians...''\\
Region, LA. & gay, jewish, trump, men, racist, homosexual, group, white, nazi, issue & ``Something gay went wrong'' \\
Region, NA. & white, homosexual, men, israel, obama, word, left, issue, pride, small & ``Absolute nonsense.  Where do you get this stuff? Trump has as much to do with White Supremacy  as Obama with radical Islamic terrorists.''\\
Region, Oc. & anti, trump, nazi, think, jew, israel, terrorist, american, white, going & ``Anti 'infidel' hate by Muslims has no place in MY Canada.''\\
Region, Si. & yes, trump, like, christian, jewish, neo, http, www, democrat, read & ``We don't need life without parole. We need the death penalty.''\\
Region, SSA. & catholic, christian, church, trump, yes, time, anti, doe, party, make & ``Catholicism certainly. They were expert terrorists.''\\
Region, WE. & white, jew, homosexual, world, human, black, race, change, gay, church & ``The underlying intent of EU is to destroy the white race, Christianity, and western civilization. Leave it.'' \\

\midrule
\bottomrule
\end{tabular}}
\caption{LEXICON}
\label{tab:lexicon}
\end{table*}


\begin{table*}[]
    \centering
    \scalebox{.75}{
    \begin{tabular}{p{15cm}p{3cm}}
    \toprule
        & Annotated as\\
        Item & offensive \\\midrule
        \multirow{4}{*}{\shortstack[l]{Transgender athletes..... Transgender students.....  This is what feminism gets you in society.\\  This was unheard of only a short 20 years ago.}} & Arab Culture, \\ & Latin America, \\ &  North America, \\ & Oceania\\ \\
        \multirow{3}{*}{\shortstack[l]{I presume a combat rosary saw service in Iraq or Afghanistan.  While Mary loves all the troops, \\ I am not sure that Mary the Palestinian Jew would approve of any foreign occupation by an\\ imperialist power, speaking of that other kind of Americanism.}} & North America, \\
        & Western Europe\\
        &\\
        \multirow{4}{*}{\shortstack[l]{A Jew can become a gentile and a gentile can become a Jew but a man cannot become a \\woman nor a woman a man.}} & Arab Culture \\
        & Latin America \\
        & North America \\
        & Western Europe \\
        \bottomrule
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
\end{comment}


\begin{table*}[]
    \centering
    \scalebox{.75}{
    \begin{tabular}{p{11cm}ccccccccc}
    \toprule
        & \multicolumn{2}{c}{Marked as} & \\\cline{2-3}
        Item & Offensive & not Offensive & Category  \\\midrule
        What's up, Doc? Don't forget the shemozzle at Red River College in Winnipeg. Nyaaah, what a maroon! & AC, LA, Oc & ICS, NA, Si, SSA, WE & random \\\\
        I bet if she was a Nun you would have more respect. & AC, LA, NA & ICS, Oc, Si, SSA, WE & Morality \\\\
        Transgender athletes..... Transgender students.....  This is what feminism gets you in society.  This was unheard of only a short 20 years ago. & AC, LA, NA, Oc & ICS, Si, SSA, WE & transgender \\\\
        Does pointing out that a growing majority of Americans support adultery (abortion, same sex marriage, even theft), change God's law an iota?&AC, ICS, LA, NA & Oc, Si, SSA, WE &LGB\\\\
        A Jew can become a gentile and a gentile can become a Jew but a man cannot become a woman nor a woman a man.&AC, LA, NA, Oc, WE & ICS, Si, SSA &jewish \\\\
        %JJ: You forgot to acknowledge that Lesbians also murder their SO's just like Hetro's, Homosexuals, and  all the other groups do,  and Democratic Men Cheat as well.  Lets not leave out any pertinent ones.......&ICS, LA& LGB\\\\
        %I can't see why.  Gay people are just as responsible as everyone else to pay the societal costs associated with unwanted pregnancies.  But I guess a hater gotta' hate.& AC, ICS, LA, NA &LGB\\\\
        
        
        %Republican party FILTHY w super fakey 'christians'.  They'll stab in you in the back for a buck, wave a flag, then kick you in the face ... & AC, ICS, LA, Oc, SSA & NA, Si, WE & christian \\\\
        The women came out because he is a hypocrite, a child predator.  Come on trumpers,  defend the child predator Christian, lol & ICS, LA, Oc, SSA & AC, NA, Si, WE& christian\\
        \bottomrule
    \end{tabular}}
    \caption{Instances with highest disagreement across regions.}
    \label{tab:items-region}
\end{table*}

==> tabs/multi-perspective.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\scalebox{.8}{
\begin{tabular}{llll}\toprule
\multicolumn{2}{c}{Annotator}             & Global &  Perspective \\
\multicolumn{2}{c}{Cluster}     & Head &  Model\\
                               \midrule
\multirow{ 8 }{*}{ Region }
& AC & 39.2 & 42.6 \\
& ICS & 36.3 & 46.4 \\
& LA & 37.8 & 36.1 \\
& NA & 37.3 & 39.8 \\
& Oc & 38.5 & 40.7 \\
& Si & 33.2 & 29.2 \\
& SSA & 34.5 & 33.4 \\
& WS & 37.4 & 33.4 \\
\midrule
& 2 & 39.7 & 53.4 \\
& 3 & 38.5 & 46.2 \\
Moral& 1 & 40.3 & 48.4 \\
Clusters& 5 & 36.0 & 32.9 \\
& 4 & 35.5 & 41.6 \\
& 0 & 37.4 & 47.9 \\
\bottomrule
\end{tabular}}
\end{table}
